Toward a Secure Crowdsourced Location Tracking System

Low-energy Bluetooth devices have become ubiquitous and widely used for different applications. Among these, Bluetooth trackers are becoming popular as they allow users to track the location of their physical objects. To do so, Bluetooth trackers are often built-in within other commercial products connected to a larger crowdsourced tracking system. Such a system, however, can pose a threat to the security and privacy of the users, for instance, by revealing the location of a user's valuable object. In this paper, we introduce a set of security properties and investigate the state of commercial crowdsourced tracking systems, which present common design flaws that make them insecure. Leveraging the results of our investigation, we propose a new design for a secure crowdsourced tracking system (SECrow), which allows devices to leverage the benefits of the crowdsourced model without sacrificing security and privacy. Our preliminary evaluation shows that SECrow is a practical, secure, and effective crowdsourced tracking solution

==> Makefile <==
# name of the tex file, without extension
FILENAME=main
BIB = *.bib
SOURCES=sections/*.tex

all: sanitize $(FILENAME).tex
	rubber -Wall --unsafe --synctex --pdf $(FILENAME) || rubber -Wall --unsafe --synctex --pdf $(FILENAME)
	rubber-info $(FILENAME)
	mv $(FILENAME).pdf crowdsourcetracking.pdf
	xdg-open crowdsourcetracking.pdf	

clean:
	rubber --clean $(FILENAME)
	rm -f output/* *.log
	rm -f $(FILENAME).pdf

sanitize:
	sed -i 's/ i\.e\./ \\ie/g' sections/*.tex
	sed -i 's/ etc\./ \\etc/g' sections/*.tex
	sed -i 's/ viz\./ \\viz/g' sections/*.tex
	sed -i 's/ e\.g\./ \\eg/g' sections/*.tex

spellcheck:
	aspell check --lang=en_US $(FILENAME).tex

loop:
	while true; do inotifywait -r -e MODIFY $(SOURCES); printf %50s |tr " " "="; echo""; make clean; make;   done

check:
	chrisper *.tex

.PHONY: all clean clean_leavepdf spellcheck pdf loop check rtf


==> sections/implementation.tex <==
\section{Preliminary Implementation}

We did a preliminary implementation of~\systemname using Raspberry Pi 3B with~\ac{BLE} as our~\ac{TD}.
We implemented python based implementations of the~\ac{CD} and~\ac{TS} functionalities.
%We developed a simple Android app to be our~\ac{TApp} that encompasses all the operations related to the~\ac{CD}.
%Our~\ac{TS} is a python-based web server.

%All the communications with~\ac{TS} are through~\ac{TLS} that ensures that that~\ac{TS} cannot be spoofed.
The~\ac{TS} knows the public keys of all~\acp{TD}.


%In order to verify \systemname{} and measure the load on data transfer, we implemented the protocol using a Raspberry Pi 3B as a functioning ~\ac{TD}. A seperate machine emulated ~\ac{CD} and ~\ac{TS}. Each entity had a (public, private) key pair of their own. And by design, ~\ac{TS} is aware of all the public keys for any given ~\ac{TD}. Both a secure version that uses encryption and an insecure version without encryption were implemented.
%
%For the secure Python based implementation we used RSA encryption using public-private key pairs generated by OpenSSL. PyBluez was used for Bluetooth sockets, and standard http sockets without TLS were used to enable communication between ~\ac{TS} and ~\ac{CD}. The insecure implementation has a similar setup without any encryption.
%
%\todocm{Cite the PyBluez library}{}
%\todocm{Image of a Raspberry Pi 3B}{}
%
%Since the secure implementation was done mainly as a proof of work to test the protocols. This meant that the code was not as optimal as it can be, and thus it leaves some room for improvement in terms of memory consumption as well as computation. And using a Raspberry Pi 3B as a ~\ac{TD} meant that the power consumption will be higher than that of a standard BLE device considering for our experiments we had networking adapters turned on for remote communication. 

==> sections/motivation.tex <==
\section{Motivation}
There are numerous crowdsourced BLE tracking devices that exist in the market. More and more manufacturers such as Apple have shown interest in making such a product that will increase the adoption of such devices and it's accompanying technology. 

To understand the current state of these devices, we analyzed some of the popular devices available in the market. However, none of these devices were secure and often times easy for an attacker to obtain and or spoof parts of the service. This causes a huge risk to the users of such devices as these devices are often used to keep track of valuable items. 

And since there have been numerous publications on the security issues with Bluetooth technology, we find that such a system requires more scrutiny regarding the threat it poses to a users privacy. 

==> sections/securityproperties.tex <==
\section{Crowdsource tracking security properties}
As mentioned before, the main goal of any crowdsourced tracking system is to provide an ability for users to know the reliable location of tracking devices.
From a security and privacy perspective, we also want certain properties to hold for any crowdsourced tracking system. 
Furthermore, for each of the properties, we identify the necessary capabilities required to satisfy the corresponding property.

All security properties are named as X-Sy, where X is the entity for which the security property belongs, and y is a number indicating a unique id.

Similarly, a capability required for a security property with name M is named as M*X-Cy, where X is the entity that needs to have the capability, and y is a number indicating a unique id.

The security properties and the corresponding required capabilities are listed below:
Tracking Device Security:
Privileged owners (TD-S1): Only owners can perform privilege operations on a tracking device. Specifically, we consider the following operations as privileged: 
	To know the location of the~\ac{TD} from the~\ac{TS}.
	To perform ringing or blinking or other actions remotely (\ie{}, through~\ac{BLE}) that bring human attention to the~\ac{TD}.

The intuition here is to ensure that only owners of a~\ac{TD} be able to access services of the~\ac{TS} w.r.t the corresponding~\ac{TD}.
Required capabilities:
    TD-S1*TD-C1: The~\ac{TD} should be able to recognize its owners.
    TD-S1*TS-C1: The~\ac{TS} should be able to recognize owners of a given~\ac{TD}.

Physical ownership (TD-S2): It should be impossible to own a tracking device without physical access.

This is based on traditional ownership requirement~\ie{} to own a device, it is important to ensure that the device can be accessed physically.

Required capabilities:
TD-S2*TD-C1: Owning of a~\ac{TD} should involve performing a physical action on the~\ac{TD}. 
TD-S2*TS-C1: The~\ac{TS} should be able to verify the proof of the physical activity on the~\ac{TD}.


Communication Device Security:

Anonymous location update (CD-S1): A~\ac{CD} should be able to~\emph{anonymously} update the location of~\emph{only} in proximity~\acp{TD} .

This ensures that participating in the crowdsource tracking system does not pose any privacy risks to the~\ac{CD}. Furthermore, ensuring that location can be updated for the only those~\acp{TD} that are in BLE proximity enabled protection against Sybil attacks (cite).

Required capabilities:

CD-S1*TS-C1: The~\ac{CD} should be able to update the location of a~\ac{TD} if and only if the~\ac{TD} is in BLE proximity or, in other words, the~\ac{CD} can communicate with the corresponding~\ac{TD}.

Tracking Service Security:
Reliable location service (TS-S1): The location information of~\acp{TD} that is provided by the~\ac{TS} should be reliable. \ie{}, location of a~\ac{TD} provided by the~\ac{TS} should indeed be the location of the~\ac{TD}.

This ensures that the location information about a~\ac{TD} provided by the~\ac{TS} is reliable and can be trusted by the owners.

Required capabilities:
    TS-S1-TD-C1: It should be impossible to spoof a given~\ac{TD}.
    TS-S1-CD-C1: It should be impossible to spoof a location by a~\ac{CD}.
    TS-S1-TS-C1: It should be impossible to spoof the~\ac{TS}.


For each of the above properties to hold, we need to have certain necessary conditions that should be satisfied. 
Specifically, these are the conditions if not satisfied, then it impossible to design a crowdsource tracking system that can achieve all the above properties.
TD-S1: 
        The~\ac{TD} should be able to recognize its owners.
        The~\ac{TS} should be able to recognize owners of a given~\ac{TD}.
TD-S2:
	Owning of a~\ac{TD} should involve performing a physical action on the~\ac{TD}. 
	The~\ac{TS} should be able to verify the proof of the physical activity on the~\ac{TD}.
CD-S1:
	The~\ac{CD} should be able to update the location of a~\ac{TD} if and only if the~\ac{TD} is in BLE proximity or, in other words, the~\ac{CD} can communicate with the corresponding~\ac{TD}.
TS-S1:
	It should be impossible to spoof a given~\ac{TD}.
	It should be impossible to spoof a location by a~\ac{CD}.
	It should be impossible to spoof the~\ac{TS}.


